On the Monitorability of Session Types, in Theory and Practice (Extended Version)

In concurrent and distributed systems, software components are expected to communicate according to predetermined protocols and APIs - and if a component does not observe them, the system's reliability is compromised. Furthermore, isolating and fixing protocol/API errors can be very difficult. Many methods have been proposed to check the correctness of communicating systems, ranging from compile-time to run-time verification; among such methods, session types have been applied for both static type-checking, and run-time monitoring. This work takes a fresh look at the run-time verification of communicating systems using session types, in theory and in practice. On the theoretical side, we develop a novel formal model of session-monitored processes; with it, we formulate and prove new results on the monitorability of session types, connecting their run-time and static verification - in terms of soundness (i.e., whether monitors only flag ill-typed processes) and completeness (i.e., whether all ill-typed processes can be flagged by a monitor). On the practical side, we show that our monitoring theory is indeed realisable: building upon our formal model, we develop a Scala toolkit for the automatic generation of session monitors. Our executable monitors can be used to instrument black-box processes written in any programming language; we assess the viability of our approach with a series of benchmarks.

==> figs/rules/composite-system.tex <==
\begin{figure}
  \small
  \centerline{
    \inference[\text{[\textsc{iSnd}]}]{P \xrightarrow{\triangleleft \texttt{l}(v)} P' & M \xrightarrow{\triangleright\texttt{l}(v)} M'}{\langle P ; M\rangle \xrightarrow{\tau} \langle P' ; M'\rangle}
    \hspace{1cm}
    \inference[\text{[\textsc{iRcv}]}]{P \xrightarrow{\triangleright\texttt{l}(v)} P' & M \xrightarrow{\triangleleft\texttt{l}(v)} M'}{\langle P ; M\rangle \xrightarrow{\tau} \langle P' ; M'\rangle}
  }\medskip
  \centerline{
    \inference[\text{[\textsc{iOut}]}]{M \xrightarrow{\envsndOP\texttt{l}(v)} M'}{\langle P ; M\rangle \xrightarrow{\envsndOP\texttt{l}(v)} \langle P ; M'\rangle}
    \hspace{1cm}
    \inference[\text{[\textsc{iIn}]}]{M \xrightarrow{\envrcvOP\texttt{l}(v)} M'}{\langle P ; M \rangle \xrightarrow{\envrcvOP\texttt{l}(v)} \langle P ; M'\rangle}
  }\medskip
  \centerline{
    \inference[\text{[\textsc{iProc}]}]{P \xrightarrow{\tau} P'}{\langle P ; M\rangle \xrightarrow{\tau} \langle P' ; M\rangle}
    \hspace{1cm}
    \inference[\text{[\textsc{iMon}]}]{M \xrightarrow{\tau} M'}{\langle P ; M\rangle \xrightarrow{\tau} \langle P ; M'\rangle}
  }
  \caption{Composite monitored system semantics.}\label{fig:composite-system}
\end{figure}


==> figs/rules/monitor-calculus.tex <==
%!TEX root=main.tex
\begin{figure}
  \small
  \textbf{Syntax}\hspace{1cm}
  %\centerline{
  \(  
    \begin{array}{r@{\hskip 2mm}r@{\hskip 2mm}c@{\hskip 2mm}l}
      \text{Monitor} & M,N & \coloneqq & \monsndk{l}{a}.M \;\vert\;\monrcv{i}{I} \;\vert\;\monout{l}{a}.M \;\vert\; \monin{i}{I}\\[1mm]
      & & & \;\vert\; \monmu{X}.M \;\vert\; X \;\vert\; \pif{A}{M}{N} \;\vert\; \pnil \;\vert\; \no{}{P} \;\vert\; \no{}{E}\\
    \end{array}
  \)
  %}
  \bigskip\\
  \textbf{Semantics}
  \medskip\\
  \centerline{
    \inference[\text{[\textsc{mSnd}]}]{}{\monsndk{l}{v}.M \xrightarrow{\monsndact{l}{v}} M}
    \hspace{0.5cm}
    \inference[\text{[\textsc{mOut}]}]{}{\monout{l}{v}.M \xrightarrow{\monoutact{l}{v}} M}
    \hspace{0.5cm}
    \inference[\text{[\textsc{mRec}]}]{}{\monmu{X}.M \xrightarrow{\tau} M[\nicefrac{\monmu{X}.M}{X}]}
  }\bigskip\\
  \centerline{
    \inference[\text{[\textsc{mRcv}]}]{}{\monrcv{i}{I} \xrightarrow{\monrcvactkNoVIdx{j}} M_{j}[\nicefrac{v}{x_j}]} $j\in I$% \,\text{ and } \, \emptyset\rightvdash v_j:\textsf{B}_j$
 % }\bigskip\\
 % \centerline{
    \hspace{0.5cm}
    \inference[\text{[\textsc{mIn}]}]{}{\monin{i}{I} \xrightarrow{\moninactk{j}} M_{j}[\nicefrac{v_{j}}{x_j}]} $j\in I$% \, \text{ and } \, \emptyset\rightvdash v_j:\textsf{B}_j$
  }\medskip\\
  \centerline{
    \inference[\text{[\textsc{mTru}]}]{A \Downarrow \textsf{tt}}{\pif{A}{M}{N} \xrightarrow{\tau} M}
    \hspace{1cm}
    \inference[\text{[\textsc{mFls}]}]{A \Downarrow \textsf{ff}}{\pif{A}{M}{N} \xrightarrow{\tau} N}
  }\bigskip\\
  % \centerline{
  %   \inference[\text{[\textsc{mRec}]}]{}{\monmu{X}.M \xrightarrow{\tau} M[\nicefrac{\monmu{X}.M}{X}]}
  % }\bigskip\\
  \textbf{Violation Semantics}
  \medskip\\
  \centerline{
    \inference[\text{[\textsc{mIV}]}]{}{\monrcv{i}{I} \xrightarrow{\monrcvactkNoVIdx{j}} \no{}{P}} $j\notin I$% \, \text{ or } \, \emptyset\nrightvdash v_j:\textsf{B}_j$
  % }\medskip\\
  % \centerline{
    \hspace{1cm}
    \inference[\text{[\textsc{mEV}]}]{}{\monin{i}{I} \xrightarrow{\moninactk{j}} \no{}{E}} $j\notin I$% \, \text{ or } \, \emptyset\nrightvdash v_j:\textsf{B}_j$
  }\medskip\\
  \caption[Monitor Syntax and Semantics]{Monitor Syntax and Semantics}\label{fig:monitor-calculus}
\end{figure}

% \fxASerror{I removed the type annotations in \Cref{fig:monitor-calculus}, and the side conditions ``$\emptyset\rightvdash v_j:\textsf{B}_j$''  in rules mRcv and mIn, and ``$\emptyset\nrightvdash v_j:\textsf{B}_j$'' in rules mIV, mEv. Double-check the proofs}

==> figs/rules/process-calculus.tex <==
%!TEX root=main.tex
\begin{figure}
  \small
  \textbf{Syntax}\hspace{1cm}
  {\(  
    \begin{array}{r@{\hskip 2mm}r@{\hskip 2mm}c@{\hskip 2mm}l}
      \text{Predicates} & A & \Coloneqq & \textsf{tt} \;\vert\; \textsf{ff} \;\vert\; v_{1} \equal\equal v_{2} \;\vert\; v_{1} >\equal v_{2} \;\vert\; A_{1}{\normalfont\textsf{ \&\& }}A_{2} \;\vert\; !A \;\vert\; \ldots\\[1mm]
      \text{Processes} & P,Q & \Coloneqq & \psndk{l}{a}.P \;\vert\;\prcv{i}{I} \;\vert\; \pmu{X}.P \;\vert\; X \;\vert\; \pif{A}{P}{Q} \;\vert\; \pnil\\
      % \;\vert\;\textbf{err}
    \end{array}
  \)}\bigskip\\
  \textbf{Semantics}
  \hspace{5mm}
  {
    \inference[\text{[\textsc{pRec}]}]{}{\mu_{X}.P \xrightarrow{\tau} P[\nicefrac{\mu_{X}.P}{X}]}
    \hspace{1.5cm}
    \inference[\text{[\textsc{pSnd}]}]{}{\psnd{}.P \xrightarrow{\sndact{l}{v}} P}
  }\\[2mm]
  \centerline{
    \inference[\text{[\textsc{pRcv}]}]{\phantom{X}}{\prcv{i}{I} \xrightarrow{\triangleright \pmsgNoVIdx{j}} P_{j}[\nicefrac{v}{x_j}]} $j\in I$
    % \hspace{0.3cm}
    % \inference[\text{[\textsc{pErr}]}]{}{\triangleright \{l_{i}(x_i:B_i).P_{i}\}_{i\in I} \xrightarrow{\triangleright\,l_{j}(v_{j})} \textbf{err}} $j\notin I$
  }\\[2mm]
  \centerline{
    \inference[\text{[\textsc{pTru}]}]{A \Downarrow \textsf{tt}}{\pif{A}{P}{Q}\xrightarrow{\tau} P}
    \hspace{1cm}
    \inference[\text{[\textsc{pFls}]}]{A \Downarrow \textsf{ff}}{\pif{A}{P}{Q}\xrightarrow{\tau} Q}
  }
  \caption[Process Calculus Syntax and Semantics]{Process Calculus Syntax and Semantics}\label{fig:process-calc-syntax-semantics}
\end{figure}

==> figs/rules/session-types-noa.tex <==
%!TEX root=main.tex
\begin{figure}
  \small
  \textbf{Syntax}\hspace{5mm}
  {\(
    \begin{array}{r@{\hskip 2mm}r@{\hskip 2mm}c@{\hskip 2mm}l}
      \text{Base types}& \textsf{B} & \Coloneqq & \normalfont{\textsf{Int}} \;\vert\; \normalfont{\textsf{Str}} \;\vert\; \normalfont{\textsf{Bool}} \;\vert\; \ldots \;\vert\; (\textsf{B},\textsf{B})
      \\[1mm]
      \text{Session types}& R,S & \Coloneqq & \underbrace{\stselNA{i}{I} \;\;\vert\;\; \stbraNA{i}{I}}_{\text{with $I \!\neq\! \emptyset$ and $\texttt{l}_i$ pairwise distinct}} \;\;\vert\;\; \strec{X}.S \;\;\vert\;\; X \;\;\vert\;\; \textsf{end} 
    \end{array}
    \)
  }
  % \smallskip
  % \textbf{Transitions}\\
  % \smallskip
  % \centerline{
  %   \inference[\text{[\textsc{sRec}]}]{}{\strec{X}.S \xrightarrow{\tau} S[\nicefrac{\strec{X}.S}{X}]}
  %   \hspace{0.6cm}
  %   \inference[\text{[\textsc{sSel}]}]{}{\stsel{i}{I} \xrightarrow{\selactk{j}} S_j} $j \in I$
  % }\smallskip\\
  % \centerline{
  %   \inference[\text{[\textsc{sBra}]}]{}{\stbra{i}{I} \xrightarrow{\braactk{j}} S_j} $j \in I$
  % }\smallskip\\

  \medskip

  \textbf{Dual types}\hspace{5mm}
  {\(
    \begin{array}{r@{\;\;}c@{\;\;}l@{\qquad}c}
    \overline{\stbraNA{i}{I}} &=& \oplus \big\{!\texttt{l}_{i}(\textsf{B}_{i}).\overline{S_{i}}\big\}_{i\in I} &
    \overline{\textsf{end}} \,=\, \textsf{end} \qquad {\overline{X}} \,=\, X\\[2mm]
    \overline{\stselNA{i}{I}} &=& \& \big\{?\texttt{l}_{i}(\textsf{B}_{i}).\overline{S_{i}}\big\}_{i\in I}&
    \overline{\strec{X}.S} \;=\; \strec{X}.\overline{S}
  \end{array}
  \)}
  \caption[Session Types Syntax, and Definition of Dual Types]{Session Types Syntax, and Definition of Dual Types.}\label{fig:session-types-noa}
\end{figure}

==> figs/rules/session-types.tex <==
%!TEX root=main.tex
\begin{figure}
  \small
  \textbf{Syntax}\\
  \centerline{\(
    \begin{array}{r@{\hskip 2mm}r@{\hskip 2mm}c@{\hskip 2mm}l}
      \text{Session types}& R,S & \Coloneqq & \stsel{i}{I} \quad\vert\quad \stbra{i}{I}\\
      &&& \;\vert\; \strec{X}.S \;\vert\; X \;\vert\; \textsf{end}
      \hspace{6mm}
      \text{\footnotesize(with $I \!\neq\! \emptyset$,\;$\texttt{l}_i$ pairwise distinct)} 
    \end{array}
    \)
  }
  \smallskip
  \textbf{Transitions}\\
  \smallskip
  \centerline{
    \inference[\text{[\textsc{sRec}]}]{}{\strec{X}.S \xrightarrow{\tau} S[\nicefrac{\strec{X}.S}{X}]}
    \hspace{0.6cm}
    \inference[\text{[\textsc{sSel}]}]{}{\stsel{i}{I} \xrightarrow{\selactk{j}} S_j} $j \in I$
  }\smallskip\\
  \centerline{
    \inference[\text{[\textsc{sBra}]}]{}{\stbra{i}{I} \xrightarrow{\braactk{j}} S_j} $j \in I$
  }\smallskip\\

  \textbf{Dual types}\\[2mm]
  \centerline{\(
    \begin{array}{r@{\;\;}c@{\;\;}l@{\qquad}c}
    \overline{\stbra{i}{I}} &=& \oplus \big\{!\texttt{l}_{i}(x_{i}:\textsf{B}_{i})[A_{i}].\overline{S_{i}}\big\}_{i\in I} &
    \overline{\textsf{end}} \,=\, \textsf{end} \qquad {\overline{X}} \,=\, X\\[2mm]
    \overline{\stsel{i}{I}} &=& \& \big\{?\texttt{l}_{i}(x_{i}:\textsf{B}_{i})[A_{i}].\overline{S_{i}}\big\}_{i\in I}&
    \overline{\strec{X}.S} \;=\; \strec{X}.\overline{S}
  \end{array}
  \)}
  \caption[Session Types Syntax Augmented with Assertions, their Transitions and Dual Types]{Session Types Augmented with Assertions: Syntax, Transitions and Duality}\label{fig:session-types}\label{fig:session-types-with-assertions}
\end{figure}

==> figs/rules/type-system-noa.tex <==
%!TEX root=main.tex
\begin{figure}
  \small
  \textbf{Identifier Typing}\hspace{2cm}
  %\bigskip\\
  %\centerline{
    \inference[\text{[\textsc{tVar}]}]{\Gamma(x)\equal \basetype}{\Gamma \rightvdash x : \basetype}
    \hspace{1cm}
    % \inference[\text{[\textsc{tPVar}]}]{\Theta(X)\equal S}{\Theta\cdot\Gamma \rightvdash X :S}
    % \hspace{0.5cm}
    \inference[\text{[\textsc{tVal}]}]{v \in \basetype}{\Gamma \rightvdash v : \basetype}
  %}
  \bigskip\\
  \textbf{Process Typing}
  \bigskip\\
  \centerline{
    \inference[\text{[\textsc{tBra}]}]{\forall i \in I \qquad \Theta\cdot\Gamma, x_i:\textsf{B}_i \rightvdash P_i:S_i}{\Theta\cdot\Gamma \rightvdash \prcv{i}{I \cup J}: \stbraNA{i}{I}}
    \hspace{1cm}
    \inference[\text{[\textsc{tRec}]}]{\Theta, X:S\cdot\Gamma\rightvdash P:S}{\Theta\cdot\Gamma \rightvdash \pmu{X}.P:S}
  }\bigskip\\
  \centerline{
    \inference[\text{[\textsc{tSel}]}]{\exists i \in I \qquad \texttt{l} \equal \texttt{l}_i \qquad \Gamma\rightvdash a:\textsf{B}_i \qquad \Theta\cdot\Gamma \rightvdash P:S_i}{\Theta\cdot\Gamma \rightvdash \psndk{l}{a}.P: \stselNA{i}{I}}
    \hspace{1cm}
    \inference[\text{[\textsc{tPVar}]}]{\Theta(X)\equal S}{\Theta\cdot\Gamma \rightvdash X :S}
  }\bigskip\\
  % \centerline{
  %   % \inference[\text{[\textsc{tUnf}]}]{P\not\equal\mu_X.Q,X&\Theta\cdot\Gamma\rightvdash P:S[\nicefrac{\textsf{rec }X.S}{X}]}{\Theta\cdot\Gamma \rightvdash P: \textsf{rec }X.S}
  % }\bigskip\\
  \centerline{
    \inference[\text{[\textsc{tIf}]}]{\Gamma\rightvdash A:\textsf{Bool}&\Theta\cdot\Gamma\rightvdash P:S & \Theta\cdot\Gamma\rightvdash Q:S}{\Theta\cdot\Gamma \rightvdash \pif{A}{P}{Q}: S}
    \hspace{1cm}
    \inference[\text{[\textsc{tNil}]}]{}{\Theta\cdot\Gamma \rightvdash \pnil: \textsf{end}}
  }
  \caption[Session Typing Rules]{Session Typing Rules.}\label{fig:session-typing-rules-noa}
\end{figure}


==> figs/rules/type-system.tex <==
%!TEX root=main.tex
\begin{figure}
  \small
  \textbf{Process Typing}
  \bigskip\\
  \centerline{
    \inference[\text{[\textsc{tBra}]}]{\forall i \in I, \exists j \in J \cdot \texttt{l}_j \equal \texttt{l}_i,\quad \textsf{B}_j\equal \textsf{B}_i,\quad\Theta\cdot\Gamma, x_j:\textsf{B}_j \rightvdash P_j:S_i,\quad \Gamma, x_j:\textsf{B}_j \rightvdash A_i:\textsf{Bool}}{\Theta\cdot\Gamma \rightvdash \prcv{j}{J}: \stbra{i}{I}}
  }\bigskip\\
  \medskip\centerline{
    \inference[\text{[\textsc{tSel}]}]{\exists i \in I \cdot \texttt{l} \equal \texttt{l}_i,\quad \Gamma\rightvdash a:\textsf{B}_i,\quad\Theta\cdot\Gamma \rightvdash P:S_i,\quad \Gamma,x_i:\basetype_i \rightvdash A_i:\textsf{Bool}}{\Theta\cdot\Gamma \rightvdash \psndk{l}{a}.P: \stsel{i}{I}}
  }\medskip\\
  \centerline{
    \inference[\text{[\textsc{tRec}]}]{\Theta, X:S\cdot\Gamma\rightvdash P:S}{\Theta\cdot\Gamma \rightvdash \pmu{X}.P:S}
    \hspace{1cm}
    \inference[\text{[\textsc{tPVar}]}]{\Theta(X)\equal S}{\Theta\cdot\Gamma \rightvdash X :S}
    % \inference[\text{[\textsc{tUnf}]}]{P\not\equal\mu_X.Q,X&\Theta\cdot\Gamma\rightvdash P:S[\nicefrac{\textsf{rec }X.S}{X}]}{\Theta\cdot\Gamma \rightvdash P: \textsf{rec }X.S}
  }\bigskip\\
  \medskip\centerline{
    \inference[\text{[\textsc{tIf}]}]{\Gamma\rightvdash A:\textsf{Bool}&\Theta\cdot\Gamma\rightvdash P:S & \Theta\cdot\Gamma\rightvdash Q:S}{\Theta\cdot\Gamma \rightvdash \pif{A}{P}{Q}: S}
    \hspace{1cm}
    \inference[\text{[\textsc{tNil}]}]{}{\Theta\cdot\Gamma \rightvdash \pnil: \textsf{end}}
  }
  \caption[Session Typing Rules with Assertion Well-Formedness Checks]{Session Typing Rules with Assertion Well-Formedness Checks.}\label{fig:session-typing-rules}
\end{figure}

